Turbo3D: Ultra-fast Text-to-3D Generation

We present Turbo3D, an ultra-fast text-to-3D system capable of generating high-quality Gaussian splatting assets in under one second. Turbo3D employs a rapid 4-step, 4-view diffusion generator and an efficient feed-forward Gaussian reconstructor, both operating in latent space. The 4-step, 4-view generator is a student model distilled through a novel Dual-Teacher approach, which encourages the student to learn view consistency from a multi-view teacher and photo-realism from a single-view teacher. By shifting the Gaussian reconstructor's inputs from pixel space to latent space, we eliminate the extra image decoding time and halve the transformer sequence length for maximum efficiency. Our method demonstrates superior 3D generation results compared to previous baselines, while operating in a fraction of their runtime.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
% start with t2i fast, t23d not efficient
Text-to-3D with diffusion models has achieved remarkable progress recently.  Methods that rely on score distillation based optimization, often suffer from long optimization time and low diversity. Another line of works employs diffusion models to generate multi-view images first and use a 3D reconstruction method to obtain 3D assets. However, due to the slow sampling nature of diffusion models, the inference speed of multi-view generation is highly limited, making the 3D generation process time-consuming. Moreover, there is no guarantee of multi-view consistency during the generation process, which is very likely to lead to inconsistency problems during reconstruction, thus influencing the final quality. 
%therefore to 
Therefore, in this paper, we study the problem of fast text-to-3D generation for producing high-quality 3D assets.

%remove distillation, mention time
The area of efficient text-to-3D generation remains largely underexplored. 
Recent methods, such as Instant3D~\cite{li2023instant3d} directly generates multi-view images in a 2$\times$2 grid format to reduce inference time, yet producing a 3D asset still takes over 20 seconds. 
Meanwhile, approaches like TripoSR~\cite{tochilkin2024triposr} leverage a fast feedforward 3D reconstructor~\cite{hong2023lrm} to produce a 3D object from a single input image.   
However, this approach is limited to objects with simpler details due to its deterministic nature and its inference time remains high due to the computational cost associated with generating the initial image. 
% At the same time, there is a line of work (TripoSR~\cite{tochilkin2024triposr}) that studies fast image-to-3D generation given a single image. However, it can only deal with objects with simple details and does not take the generation cost of the input image into account.
Recently, substantial progress has been made in reducing inference time by distilling diffusion models into one-step or few-step generators~\cite{salimans2022progressive,song2023consistency,yin2024one,sauer2024fast}. 
While these techniques significantly accelerate 2D image generation, effectively adapting them for multi-view 3D generation remains an open problem.
%are not well studied for the multi-view generation problem. 

%adapt distillation to mv gen, mention time
In this paper, we propose \ours, a novel ultra-fast feed-forward method composed of a few-step multi-view diffusion model and a reconstruction model, that generates high-quality 3D assets conditioned on the text prompt. 

% not full coverage
We first train a multi-step text-to-multi-view diffusion model based on the DiT architecture~\cite{peebles2023scalable}, which serves as our teacher model. 
Then we distill the multi-view diffusion model into a much faster 4-step generator using the distribution matching distillation (DMD) loss~\cite{yin2024one}.
%apply distribution matching distillation (DMD) in the multi-view generator to obtain a faster model. 
However, we find that directly applying DMD loss leads to significant quality degradation, as it fails to capture the full range of modes present in the multi-view teacher model.
%a highly degraded quality result since it can not guarantee full coverage of modes from the teacher model. 
Therefore, we propose a dual-teacher strategy for distilling multi-view generators. 
In particular, both single-view and multi-view teacher models are employed to guide the student generator's training, %for learning the distribution matching, 
where multi-view DMD loss focuses on learning consistency across multi-view images, and single-view DMD loss focuses on image quality. \tianwei{it might be helpful for some further clarifications. single-view teacher are trained on much larger set of high quality aesthetic images, which serves as a much better teacher for improving the image quality.}

% During the multi-view generation process of our distilled model, multi-view consistency is not ensured, which makes it difficult for the reconstruction model to output a high-quality 3D result. 
% Thus, we propose a self-supervised rendering loss to further improve the compatibility of our generator and the reconstruction model. 
% In particular, during distillation, we let our multi-view generator output 8 views in total, where 4 views are used as the input to the reconstruction model and the other 4 are treated as the target views. We jointly train the few-step multi-view generation model and the reconstruction model.
However, during the multi-view generation process of our distilled model, multi-view consistency is not inherently ensured, which makes it difficult for the reconstruction model to produce high-quality 3D results. 
To mitigate this issue, we propose a self-supervised rendering loss to improve the compatibility between our generator and the reconstruction model. \shubham{We don't have this self-supervised loss in the final model, right?} Specifically, during distillation, our multi-view generator outputs a total of eight views: four are used as inputs to the reconstruction model, and the other four serve as target views. By jointly training the few-step multi-view generation model and the reconstruction model, we enhance both the consistency across views and the overall quality of the reconstructed 3D assets.

We train our model on the subset of Objaverse dataset~\cite{deitke2023objaverse, deitke2024objaverse}, which contains about 400k instances with Cap3D text captions~\cite{luo2024scalable}. As a result, our proposed \ours\ is able to produce high-quality 3D assets in less than one second, and also achieves comparable quality with previous state-of-the-arts.
